ADI: Adversarial Dominating Inputs in Vertical Federated Learning Systems

Vertical federated learning (VFL) system has recently become prominent as a concept to process data distributed across many individual sources without the need to centralize it. Multiple participants collaboratively train models based on their local data in a privacy-aware manner. To date, VFL has become a de facto solution to securely learn a model among organizations, allowing knowledge to be shared without compromising privacy of any individuals. Despite the prosperous development of VFL systems, we find that certain inputs of a participant, named adversarial dominating inputs (ADIs), can dominate the joint inference towards the direction of the adversary's will and force other (victim) participants to make negligible contributions, losing rewards that are usually offered regarding the importance of their contributions in federated learning scenarios. We conduct a systematic study on ADIs by first proving their existence in typical VFL systems. We then propose gradient-based methods to synthesize ADIs of various formats and exploit common VFL systems. We further launch greybox fuzz testing, guided by the saliency score of ``victim'' participants, to perturb adversary-controlled inputs and systematically explore the VFL attack surface in a privacy-preserving manner. We conduct an in-depth study on the influence of critical parameters and settings in synthesizing ADIs. Our study reveals new VFL attack opportunities, promoting the identification of unknown threats before breaches and building more secure VFL systems.

==> alluppermath-notations.tex <==
%{math-notations}

% natural numbers
\newcommand{\NATURALS}{{\rm Nat}}

% functions names inside of math environment
\newcommand{\fun}[1]{\hbox{\it #1\/}}

% brackets that surround syntax (as in denotational semantics)
\newcommand{\synbracket}[1]{[\![{#1}]\!]}

% logic
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\DEF}{\stackrel{{\rm def}}{=}}
\newcommand{\DEFEQUIV}{\stackrel{{\rm def}}{\equiv}}
\newcommand{\DEFIFF}{\stackrel{{\rm def}}{\IFF}}

% lambda calculus
\newcommand{\LAMBDA}[1]{\lambda{#1}\:.\:}
\newcommand{\FREEVARS}[1]{{\it FV\/}\synbracket{#1}}	% free variables
\newcommand{\FREEIDS}[1]{{\it FreeIds\/}(#1)}	% free identifiers
\newcommand{\SYNTAXWITHFOR}[3]{[#2/#3]#1}	% subst #2 for #3 in #1
\newcommand{\WITHFOR}[3]{#1[#2/#3]}		% subst #2 for #3 in #1
\newcommand{\BETAREDUCESTO}{\stackrel{\beta}{\Rightarrow}}
\newcommand{\ETAREDUCESTO}{\stackrel{\eta}{\Rightarrow}}
\newcommand{\DELTAREDUCESTO}{\stackrel{\delta}{\Rightarrow}}
\newcommand{\BETAEQUALS}{\stackrel{\beta}{=}}
\newcommand{\ETAREQUALS}{\stackrel{\eta}{=}}
\newcommand{\DELTAEQUALS}{\stackrel{\delta}{=}}

% higher order lambda calculus
\newcommand{\POLY}[1]{\Lambda{#1}\:.\:}
\newcommand{\ALLTYPE}[1]{\forall{#1}\:.\:}
\newcommand{\EXISTSTYPE}[1]{\exists{#1}\:.\:}
\newcommand{\DEPFUNTYPE}[1]{\Pi{#1}\:.\:}
\newcommand{\DEPSUMTYPE}[1]{\Sigma{#1}\:.\:}

% recursion theory
\newcommand{\ZEROORMORE}[1]{{#1}^{\rm *}}
\newcommand{\ONEORMORE}[1]{{#1}^{+}}

% category theory
\newcommand{\DOM}[1]{{\it Domain\/}(#1)}
\newcommand{\POWERSET}[1]{{\it PowerSet\/}(#1)}

% topology
\newcommand{\CLOSURE}[1]{\overline{#1}}
\newcommand{\LUB}{{\rm lub}}			% least upper bound

% set theory
\def\elem{\hbox{\raise.13ex\hbox{$\scriptstyle\in$}}}
\newcommand{\GRAPH}{{\it graph}}

% relations
\newcommand{\RELATIONTYPE}[1]{2^{(#1)}}


==> calculation.tex <==
% $Id: calculation.tex 2 2008-12-23 22:46:05Z gary.leavens $
%
% Calculational proofs, a la Dijkstra, Gries, Back and von Wright, etc.
% See: David Gries, "Teaching Calculation and Discrimination:
%      A More Effective Curriculum", CACM 34(3):44-55, Mar. 1991.
% and
%      Ralph-Johan Back and Joakim von Wright,
%      "Refinement Calculus: A Systematic Introduction",
%      Springer-Verlag, 1998.
%
% AUTHOR: Gary T. Leavens

% EXAMPLES
%
% A simple example of the use of these macros is as follows.
%
% \begin{calculation}
% \FORMULA{\vec{RD}}
% \EQREASON{definition of $\vec{RD}$}
% \FORMULA{(RD_1, \ldots, RD_j, \ldots, RD_{12})}
% \REASON{\sqsubseteq}{$F_j$ is monotonic}
% \FORMULA{(RD_1, \ldots, F_j(\vec{RD}), \ldots, RD_{12})}
% \EQREASON{definition of $\vec{RD'}$}
% \LASTFORMULA{\vec{RD'}}
% \end{calculation}
%
% The following is a slightly more advanced example.
%
% \begin{calculation}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^n(\vec{\emptyset})}}
% \EQREASON{assumption $F^n(\vec{\emptyset}) = F^{n+1}(\vec{\emptyset})$}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^{n+1}(\vec{\emptyset})}}
% \EQREASON{definition of iteration of a function}
% \FORMULA{F(\vec{RD'}) \sqsubseteq F(F^n(\vec{\emptyset}))}
% \REASON{\impliedby}{monotonicity of $F$}
% \FORMULA{\vec{RD'} \sqsubseteq F^n(\vec{\emptyset})}
% \REASON{\impliedby}{transitivity}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})
%         \wedge F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})}
% \EQREASON{assumption $F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})$}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})}
% \REASON{\impliedby}{Lemma~7}
% \QEDFORMULA{\vec{RD} \sqsubseteq F(\vec{RD})}
% \end{calculation}
%
% An much more sophisticated example, with subdeductions a la Back and
% von Wright is the following.
%
% \begin{calculation}
% \FORMULA{\alpha(\{tr: (z, \ell') \mid tr \in \gamma(RD_k)\}) }
% \EQREASON{definition of $\alpha$}
% \FORMULA{\{(x, SRD(tr')(x))
%              \mid x \in \textrm{dom}(tr')
%                   \wedge tr' \in \{tr: (z, \ell') \mid tr \in \gamma(RD_k)\} \} }
% \EQREASON{set theory
%          ($tr'$ ranges over $tr: (z, \ell')$ for $tr \in \gamma(RD_k)$)}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                    \FOCUS{tr \in \gamma(RD_k)} \} }
% \EQREASON{definition of $\gamma$}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
% \EQREASON{set theory}
% \FORMULA{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%         \cup \:
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array}
%         }
% \EQREASON{focusing on the second set}
% \SUBDEDUCTION{
%      \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{set theory}
%   \FORMULA{\{(z, \FOCUS{SRD(tr: (z, \ell'))(z)}) 
%              \mid z \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(z, \ell') 
%              \mid \FOCUS{z \in \textrm{dom}(tr: (z, \ell'))},
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k)
%              \} }
%   \EQREASON{definition of $\textrm{dom}$}
%   \FORMULA{\{(z, \ell') 
%              \mid (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $\gamma$}
%   \FORMULA{\{(z, \ell') \mid tr \in \gamma(RD_k) \} }
%   \EQREASON{$tr$ can be constructed by writing the pairs of
%              $\gamma(RD_k)$ in some order}
%   \FORMULA{\{(z, \ell') \} }
% \CONCLUDE{
%    \begin{array}{l}
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array} \\
%     \cup \: \{(z, \ell')\}
%    \end{array}
%     }
% \EQREASON{focusing on the first set}
% \SUBDEDUCTION{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(x, SRD(tr)(x))
%              \mid x \neq z, x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
%   \EQREASON{set theory and the range of $SRD$}
%   \FORMULA{\begin{array}{l}
%              \{(x, SRD(tr)(x))
%                       \mid x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%            \setminus \: \{(z, \ell) \mid \ell \in \Lab\}
%            \end{array}
%           }
%   \EQREASON{Lemma \ref{lemma:simplifyToRD}}
%   \FORMULA{RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\}}
% \LASTCONCLUDE{(RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\})
%            \cup \{(z, \ell')\}}
% \end{calculation}


%%%%%%% The macros themselves follow %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% You may want to define the following with \renewcommand...

% Brackets around normal and fixed width reasons
\newcommand{\LEFTREASONBRACKET}{\langle}
\newcommand{\RIGHTREASONBRACKET}{\rangle}
% Brackets for long reasons
\newcommand{\LONGLEFTREASONBRACKET}{\left\LEFTREASONBRACKET}
\newcommand{\LONGRIGHTREASONBRACKET}{\right\RIGHTREASONBRACKET}
% width of long and fixed width reasons
\newcommand{\LONGREASONWIDTH}{5.4in}
\newcommand{\FIXEDWIDTHREASONWIDTH}{\LONGREASONWIDTH}
% The phrase that starts each reason
\newcommand{\BYPHRASE}{by~}
% Provability symbol
\newcommand{\PROVABILITYSYMBOL}{\vdash}
% Has type symbol
\newcommand{\CALCULATIONHASTYPE}{:}
% Subdeduction symbols a la Back and von Wright
\newcommand{\SUBDEDUCTIONMARKER}{\bullet}
\newcommand{\CONCLUDEMARKER}{\cdot}

% The macros below assume that you have defined \QED,
% e.g., as \newcommand{\QED}{q.e.d.}


%%% The rest shouldn't usually need to be redefined

% The main environment
\newenvironment{calculation}{
\samepage
\begin{tabbing}
n \= n \= n \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= \kill
}{
\end{tabbing}
}

% Use for the last formula (to avoid extra vertical space)
\newcommand{\LASTFORMULA}[1]{\> \ensuremath{#1}}
% Use for the last formula in a proof that concluses the proof
\newcommand{\QEDATEND}{~~\QED}
\newcommand{\QEDFORMULA}[1]{\LASTFORMULA{#1\QEDATEND}}

% All other formulas in a calculation
\newcommand{\FORMULA}[1]{\LASTFORMULA{#1} \\}

% Generic reason, with connective and the justification
\newcommand{\REASON}[2]{%
    \ensuremath{#1}\> \>
       \mbox{\ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}#2\ensuremath{\RIGHTREASONBRACKET}} \\}

% Reasons with longer justifications, with the right bracket at the end
\newcommand{\FIXEDWIDTHREASON}[2]{%
     \ensuremath{#1}\> \>
       \ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}%
       \parbox[t]{\FIXEDWIDTHREASONWIDTH}{#2\ensuremath{\RIGHTREASONBRACKET}}
       \\
     }

% Reasons with longer justifications, with big brackets around the reason
\newcommand{\LONGREASON}[2]{%
    \ensuremath{#1}\> \>
      \ensuremath{\LONGLEFTREASONBRACKET
                  \parbox[c]{\LONGREASONWIDTH}{{\BYPHRASE}#2}
                  \LONGRIGHTREASONBRACKET
                 }
      \\
    }

% Specialization of reasons to equality
\newcommand{\EQREASON}[1]{\REASON{=}{#1}}
\newcommand{\EQLONGREASON}[1]{\LONGREASON{=}{#1}}
\newcommand{\EQFIXEDWIDTHREASON}[1]{\FIXEDWIDTHREASON{=}{#1}}

% Use \FOCUS{E} to say that subformula E will be changed in the following step
\newcommand{\FOCUS}[1]{\mbox{``}#1\mbox{''}}


%% The following are for Back and von Wright style calculations.
%% First time users may want to ignore these.

% Use for assumptions in a type-deduction style proof
\newcommand{\GIVEN}[1]{\FORMULA{#1}}
% Use \PROVETHAT to start the body of a type-deduction style proof.
\newcommand{\PROOFLINE}[2]{\ensuremath{#1} \> \ensuremath{#2} \\}
\newcommand{\PROVETHAT}[1]{\PROOFLINE{\PROVABILITYSYMBOL}{#1}}
%% Subdeductions
% Use to start a subdeduction
\newcommand{\SUBDEDUCTION}[1]{\+\+\kill\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to separate one subdeduction from another
\newcommand{\ANDALSO}{\-\-\kill}
% Use to start the next subdeduction after \ANDALSO
\newcommand{\NEXTDEDUCTION}[1]{\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to conclude a subdeduction 
\newcommand{\CONCLUDE}[1]{\-\-\kill\PROOFLINE{\CONCLUDEMARKER}{#1}}
% Use when the last formula is also a conclusion
\newcommand{\LASTCONCLUDE}[1]{\-\-\kill\ensuremath{\CONCLUDEMARKER} \> \ensuremath{#1}}
% Use in a type-deduction proof instead of \REASON, to give the rule name
\newcommand{\TYPINGRULE}[1]{\ensuremath{\CALCULATIONHASTYPE} \> ~~~ #1 \\}

% end of calculation.tex


==> denotational-semantics.tex <==
% requires math-notations

% Typography as in Schmidt's book: Denotational Semantics.
% Many of the following defs must be used in a math environment; all can be.

% natural numbers: \NATURALS
\renewcommand{\NATURALS}{{\it Nat}}
\newcommand{\ZERO}{{\it zero}}
\newcommand{\ONE}{{\it one}}
\newcommand{\TWO}{{\it two}}
\newcommand{\THREE}{{\it three}}
\newcommand{\FOUR}{{\it four}}
\newcommand{\PLUS}{{\it plus}}
\newcommand{\MINUS}{{\it minus}}
\newcommand{\TIMES}{{\it times}}
\newcommand{\EQUALNATURALS}{{\it equals}}

% integers: \INTEGER
\newcommand{\INTEGER}{{\it Int}}
\newcommand{\ADDR}{{\it Addr}}

% Booleans: \BOOLEAN
\newcommand{\BOOLEAN}{{\it Boolean}}
\newcommand{\TRUE}{{\it true}}
\newcommand{\FALSE}{{\it false}}
\newcommand{\NOT}{{\it not}}
\newcommand{\OR}{{\it or}}
\newcommand{\AND}{{\it and}}
\newcommand{\IFEXP}[3]{#1 \rightarrow #2 [\!] #3 }
\newcommand{\IFHEAD}[1]{#1 \rightarrow}
\newcommand{\IFELSE}{[\!]~}

% truth values
\newcommand{\TR}{{\it Tr}}
\newcommand{\TT}{{\it tt}}
\newcommand{\FF}{{\it ff}}

% Strings: \STRING
\newcommand{\STRING}{{\it String}}
\newcommand{\EMPTYSTRING}{{\it empty}}
\newcommand{\ERRORSTRING}{{\it error}}
\newcommand{\CONCATSTRINGS}{{\it concat}}
\newcommand{\LENGTHOFSTRING}{{\it length}}
\newcommand{\SUBSTRING}{{\it substr}}		% 3 arguments

% other primitive domains
\newcommand{\UNIT}{{\it Unit}}
\newcommand{\ERROR}{{\it Error}}

% other standard semantics domain names
\newcommand{\ANSWERS}{{\it Answer}}
\newcommand{\CMDCONT}{{\it Cmdcont}}
\newcommand{\DENOTABLE}{\mbox{\it Denotable-value}}
\newcommand{\ENVIRONMENT}{{\it Environment}}
\newcommand{\EXPRESSIBLE}{\mbox{\it Expressible-value}}
\newcommand{\EXPCONT}{{\it Expcont}}
\newcommand{\LOCATION}{{\it Location}}
\newcommand{\PROCEDURE}{{\it Procedure}}
\newcommand{\REFERENCE}{{\it Reference}}
\newcommand{\RESULT}{{\it Result}}
\newcommand{\STORE}{{\it Store}}
\newcommand{\STORABLE}{\mbox{\it Storable-value}}
\newcommand{\UNBOUND}{{\it Unbound}}
\newcommand{\VALUE}{{\it Value}}

% disjoint union: $A + B$
\newcommand{\INJECTION}[1]{{\rm in}\!{#1}}
\newcommand{\ISTEST}[1]{{\rm is}\!{#1}}
\newcommand{\CASEHEAD}[1]{\mbox{{\bf cases} ${#1}$ {\bf of} }}
\newcommand{\CASE}[2]{{#1} \:\rightarrow\: {#2}}
\newcommand{\CASESEP}{[\!]}
\newcommand{\CASEELSE}{\mbox{{\bf else} }}
\newcommand{\CASEEND}{{\bf end}}

% product space: $A \times B$
\newcommand{\PAIR}[2]{({#1},{#2})}
\newcommand{\FST}{{\it fst}}
\newcommand{\SND}{{\it snd}}
\newcommand{\ATINDEX}[2]{#1 \downarrow #2}
% Note $\ZEROORMORE{A} = Unit + A + (A \times A) + (A \times A \times A) + ...$
% Lists are $Unit + A + (A \times A) + (A \times (A \times A)) + ...$

% list space: $\LIST{A}$
\newcommand{\LIST}[1]{{\it List}(#1)}
\newcommand{\LNIL}{{\it nil}}
\newcommand{\LCONS}{{\it cons}}
\newcommand{\LHEAD}{{\it hd}}
\newcommand{\LTAIL}{{\it tl}}
\newcommand{\LNULL}{{\it null}}

% function space: $A \rightarrow B$
\newcommand{\UPDATEFUN}[3]{[{#1} \mapsto {#2}]{#3}}

% finite functions
\newcommand{\FINITEARROW}{\stackrel{{\rm fin}}{\rightarrow}}

% lifted domain: $\LIFT{A}$
\newcommand{\LIFT}[1]{{#1}_{\bot}}
\newcommand{\STRICTLAMBDA}[1]{\underline{\lambda}{#1}\:.\:}
\newcommand{\LETHEAD}[2]{\mbox{{\bf let} }{#1} = {#2}\mbox{ {\bf in} }}
\newcommand{\MAP}[2]{\mbox{{\bf map} }{#1} => {#2\{#1\}}}

% fixpoints
\newcommand{\FIX}{{\it fix}}

% common valuation functions
\newcommand{\MEANING}[2]{{\cal #1}\synbracket{#2}}
\newcommand{\DENEXPRESSION}[1]{\MEANING{E}{#1}}
\newcommand{\DENCOMMAND}[1]{\MEANING{C}{#1}}
\newcommand{\DENLITERAL}[1]{\MEANING{L}{#1}}
\newcommand{\DENPROGRAM}[1]{\MEANING{P}{#1}}

% an environment for typesetting
\newenvironment{DENOTATIONAL}{%
\samepage
\begin{tabbing}
mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= mmm \= \kill
}{
\end{tabbing}
}


==> grammar.tex <==
%{grammar}, needs {obey}

%\newcommand{\heading}[1]{\vspace{3ex}{\noindent#1}\vspace{1.5ex}}
\newcommand{\goesto}{\mbox{$::=$}}
\newcommand{\arbno}[1]{#1\hbox{\rm*}}
\newcommand{\nonterm}[1]{\mbox{$\langle$#1$\rangle$}}

\newenvironment{grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{mathGrammar}{
  \def\:{\goesto{}}
  \def\|{\hbox{$\vert$}}
   \begin{displaymath}%
     \tt \obeyspaces%
}%
{\unskip\end{displaymath}}

% Commented grammars

% length before comments start on right
\newlength{\BEFOREGRAMCOMMENTLEN}
\setlength{\BEFOREGRAMCOMMENTLEN}{7cm}

% style of text inside quotations
\newcommand{\GRAMCOMMENTSTYLE}[1]{\texttt{#1}}

\newenvironment{commented-grammar}{%
\begin{grammar}%
\qquad \= $\vert$ \= \qquad \hspace*{\BEFOREGRAMCOMMENTLEN} \= \kill%
}{%
\end{grammar}%
}

\newcommand{\gramcomment}[1]{\textrm{``\GRAMCOMMENTSTYLE{#1}''}}


==> model-structure.tex <==
\section{Learning Protocol Setup Details}
\label{sec:protocol-setup}

\smallskip

We report detailed setup of all VFL models in \T~\ref{tab:modeldetails},
including the architectures, feature partitions and number of data samples
within each dataset. The NUS-WIDE and MNIST datasets are processed by the
SplitNN learning protocol while Credit and Vehicle are processed by HeteroLR. As
for the VQA v2.0 dataset, we extend the state-of-the-art VQA framework, Oscar,
which processes the image and text features using FasterRCNN and BERT,
respectively. Users can refer to the reported information as well as our
released scripts for implementation details and further
extension~\cite{snapshot}.

\begin{table*}[t]
	\centering
	\scriptsize
  \caption{VFL model setup details under various settings over two participants \ma\ and \mb.}
	\label{tab:modeldetails}
	\resizebox{1.00\linewidth}{!}{
		\begin{tabular}{|l|c|c|c|c|c|c|c|}
			\hline
      \multirow{2}{*}{\textbf{Dataset}}  & \multirow{2}{*}{\textbf{\#Cases}} & \multirow{2}{*}{\textbf{Learning Protocol}} & \multicolumn{2}{|c|}{\textbf{Participant \ma}} & \multicolumn{2}{|c|}{\textbf{Participant \mb}} & \multirow{2}{*}{\textbf{Central Coordinator \mc}} \\\cline{4-5}\cline{6-7}
                                         &                                   &                                             & \textbf{\#Partitioned Features} & \textbf{Setup} & \textbf{\#Partitioned Features} & \textbf{Setup} & \\
			\hline
			\textbf{NUS-WIDE} & 269,648  & SplitNN  & 634 & 2-FCs with ReLU & 1,000 & 2-FCs with ReLU & 2-FCs with ReLU \\
			\textbf{Credit}   & 30,000   & HeteroLR & 13  & 1-FC & 10 & 1-FC & Sigmoid \\
			\textbf{Vehicle}  & 946      & HeteroLR &  9  & 1-FC &  9 & 1-FC & Sigmoid \\
			\textbf{MNIST}    & 60,000   & SplitNN  & 14 $\times$ 28 pixels & 3-Convs with ReLU & 14 $\times$ 28 pixels & 3-Convs with ReLU & 1-FC with ReLU \\
			\textbf{VQA v2.0}  & 82,783    & VFVQA    & 2,054 & FasterRCNN~\cite{ren2016faster} & 128 $\times$ 512 word embedding & BERT~\cite{li2020oscar} & Multi-Layer Transformers \\
			\hline
		\end{tabular}
	}
\end{table*}


==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}


==> proof-cor1.tex <==
\subsection{Proof of Corollary~\ref{cor:adi-in-VFLR}}
\label{sec:cor1}

% \textbf{Corollary~\ref{cor:adi-in-VFLR}} (Variance of HeteroLR).
% With fixed input $X_{\mathcal{A}}^*$ and varying input $X_{\mathcal{B}}$ following any distribution whose density function is $p(X_{\mathcal{B}})$, the output variance of HeteroLR is:

% \setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
% \setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
% \scriptsize
% \begin{equation*}
%     \begin{aligned}
%         \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (f(X_{\mathcal{A}}^*, X_{\mathcal{B}})) & = \sum_{k=1}^{\mathcal{K}}  \, - \frac{\pi_k}{\sqrt{2\pi}} \frac{1}{\sqrt{\sigma_k'^2 + \sigma_2^2}} \exp\{ -\frac{1}{2} \frac{\mu_k'^2}{\sigma_k'^2 + \sigma_2^2} \}\\
%         + & \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sqrt{\sigma_1^{2} + \sigma_k'^2}}) (1 -  \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sqrt{\sigma_1^{2} + \sigma_k'^2}})) \; ,
%     \end{aligned}
% \end{equation*}
% \normalsize
% \noindent where the density function $p(X_{\mathcal{B}})$ is approximated by Gaussian Mixture Model: $p(X_{\mathcal{B}}) \approx \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(X_{\mathcal{B}} | \boldsymbol{\mu_k}, \boldsymbol{\Sigma_k})$, $ \sum_{k=1}^{\mathcal{K}} \pi_k = 1$, $ \pi_k > 0 $, $\mathcal{K}$ is a finite number, $\boldsymbol{\mu_k} \in \mathbb{R}^{d_2}$, $\boldsymbol{\Sigma_k} \in \mathbb{R}^{d_2 \times d_2}$, $\mu_k' = \theta_{\mathcal{A}}^T \, X_{\mathcal{A}}^* + \theta_{\mathcal{B}}^T \, \boldsymbol{\mu_k}$, $\sigma_k'^2 = \theta_{\mathcal{B}}^T \, \boldsymbol{\Sigma_k} \, \theta_{\mathcal{B}}$, $\sigma_1 = 1.699$, and $\sigma_2 = 1.630$.

\begin{proof}
Considering the fixed input $X_{\mathcal{A}}^*$ and varying input $X_{\mathcal{B}}$, and let $ S = \theta_{\mathcal{A}}^T
\, X_{\mathcal{A}}^* + \theta_{\mathcal{B}}^T \, X_{\mathcal{B}} $. Thus, $f(X_{\mathcal{A}}^*, X_{\mathcal{B}}) = g(S)$.
Aligned with the conventions~\cite{lee2017deep, makhzani2015adversarial, hjelm2018learning, belghazi2018mutual, fei2006one, zhu1996region} in machine learning, we use Gaussian mixture model~\cite{mclachlan1988mixture} and Expectation Maximization~\cite{dempster1977maximum} to approximate the density function $p(X_{\mathcal{B}})$. Note that GMMs can approximate any smooth distributions~\cite{goodfellow2016deep}.

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        p(X_{\mathcal{B}}) \approx \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(X_{\mathcal{B}} | \boldsymbol{\mu_k}, \boldsymbol{\Sigma_k}) \; ,
    \end{aligned}
\end{equation}
\normalsize
\noindent where $ \sum_{k=1}^{\mathcal{K}} \pi_k = 1$, $ \pi_k > 0 $, $\mathcal{K}$ is a finite number, $\boldsymbol{\mu_k} \in \mathbb{R}^{d_2}$ and $\boldsymbol{\Sigma_k} \in \mathbb{R}^{d_2 \times d_2}$.
If $p(X_{\mathcal{B}})$ is discrete and not smooth (e.g. $X_{\mathcal{B}}$ is categorical data), we can approximate it by taking $\boldsymbol{\Sigma_k} \rightarrow \boldsymbol{0}$ and $\mathcal{K}$ becomes the total number of distinct data in $X_{\mathcal{B}}$, the Gaussian distribution density would become a Dirac delta function~\cite{dirac1981principles} and the following calculations still hold. 

Further, we can obtain the
density function of $S$ as: $ p(S) = \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(S | \theta_{\mathcal{A}}^T \, X_{\mathcal{A}}^* + \theta_{\mathcal{B}}^T \,
\boldsymbol{\mu_k}, \theta_{\mathcal{B}}^T \, \boldsymbol{\Sigma_k} \, \theta_{\mathcal{B}}) $. Taking $\mu_k'
= \theta_{\mathcal{A}}^T \, X_{\mathcal{A}}^* + \theta_{\mathcal{B}}^T \, \boldsymbol{\mu_k}$ and $\sigma_k'^2 =
\theta_{\mathcal{B}}^T \, \boldsymbol{\Sigma_k} \, \theta_{\mathcal{B}}$, we thus calculate the expected value of
the output:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{E}&_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (g(S)) 
        = \int g(t) \, \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(t | \mu_k', \sigma_k'^2) \, dt \\
        &\approx \int \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{t}{\sigma_1}) \, \mathcal{N}(t| \mu_k', \sigma_k'^2) \, dt
        = \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sqrt{\sigma_1^{2} + \sigma_k'^2}})
        \label{formula:sig-expectation}
    \end{aligned}
\end{equation}
\normalsize
\noindent Here, the $g(t)$ is approximated by the cumulative distribution function of standard Gaussian distribution and parameter $\sigma_1$ as $\Phi(\frac{t}{\sigma_1})$, where $\sigma_1 = 1.699$ to minimize the $L_2$ error. 
%
The variance of the output is calculated as follows:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (g(S)) 
        &= \left \langle g(S)^2 \right \rangle - \left \langle g(S) \right \rangle^2 \\
        &= \left \langle g(S) - g(S)(1-g(S)) \right \rangle - \left \langle g(S) \right \rangle^2 \\
        &= \left \langle g(S) \right \rangle (1 - \left \langle g(S) \right \rangle) - \left \langle g'(S) \right \rangle \; ,
        \label{formula:sig-variance}
    \end{aligned}
\end{equation}
\normalsize
where $\left \langle \cdot \right \rangle$ donates $\mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} ( \cdot )$. Further, we approximate the derivation of Sigmoid function $g'(S)$ using the pdf of Gaussian distribution. 
When the $L_2$ error is minimized, we get the approximated function of $g'(S)$ with $\sigma_2 = 1.630$:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        g'(S) \approx \frac{1}{\sqrt{2\pi}\sigma_2} \exp\{-\frac{S^2}{2\sigma_2^2}\}
    \end{aligned}
\end{equation}
\normalsize

Further, we can calculate the expected value of the derivation of Sigmoid function:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \label{formula:derivation-sigmoid-expectation}
        \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (g'(S)) &= \int \sum_{k=1}^{\mathcal{K}} \, \frac{\pi_k}{2\pi\sigma_k'\sigma_2} \exp\{ -\frac{t^2}{2\sigma_2^2} - \frac{(t - \mu_k')^2}{2\sigma_k'^2} \} dt \\
        &= \sum_{k=1}^{\mathcal{K}} \, \frac{\pi_k}{\sqrt{2\pi}} \frac{1}{\sqrt{\sigma_k'^2 + \sigma_2^2}} \exp\{ -\frac{1}{2} \frac{\mu_k'^2}{\sigma_k'^2 + \sigma_2^2} \}
    \end{aligned}
\end{equation}
\normalsize

According to \E~\ref{formula:sig-expectation}, \E~\ref{formula:sig-variance} and \E~\ref{formula:derivation-sigmoid-expectation}, we can calculate the variance of logistic regression result as follows:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} & (g(S)) = \,\sum_{k=1}^{\mathcal{K}}  \, - \frac{\pi_k}{\sqrt{2\pi}} \frac{1}{\sqrt{\sigma_k'^2 + \sigma_2^2}} \exp\{ -\frac{1}{2} \frac{\mu_k'^2}{\sigma_k'^2 + \sigma_2^2} \}\\
        & + \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sqrt{\sigma_1^{2} + \sigma_k'^2}}) (1 -  \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sqrt{\sigma_1^{2} + \sigma_k'^2}}))
    \end{aligned}\qedhere
\end{equation}
\normalsize

\end{proof}

==> proof-cor2.tex <==
\subsection{Proof of Corollary~\ref{cor:adi-in-VFNN}}
\label{sec:cor2}

% \textbf{Corollary~\ref{cor:adi-in-VFNN}} (Variance of SplitNN).
% With fixed input $X_{\mathcal{A}}^*$ and varying input $X_{\mathcal{B}}$ following any distribution whose density function is $p(X_{\mathcal{B}})$, the output variance of SplitNN is:

% \scriptsize
% \setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
% \setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
% \begin{equation*}
%     \begin{aligned}
%         \mathbb{V}&_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (f(X_{\mathcal{A}}^*,X_{\mathcal{B}}))\\
%         & = (\sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'})) \, 
%         (\sum_{k=1}^{\mathcal{K}} \pi_k^2 \, \sigma_k'^2(1 - \frac{\mu_k'}{\sigma_k'} \frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})} - (\frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})})^2) \\
%         & \; + (\sum_{k=1}^{\mathcal{K}} \pi_k \, (\mu_k' + \sigma_k' \frac{\phi(\frac{\mu_k'}{\sigma'_k})}{\Phi(\frac{\mu_k'}{\sigma_k'})}))^2
%         (1 - \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'}))) \; ,
%     \end{aligned}
% \end{equation*}
% \normalsize
% \noindent where the density function $p(X_{\mathcal{B}})$ is approximated by Gaussian Mixture Model: $p(X_{\mathcal{B}}) \approx \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(X_{\mathcal{B}} | \boldsymbol{\mu_k}, \boldsymbol{\Sigma_k})$, $ \sum_{k=1}^{\mathcal{K}} \pi_k = 1$, $ \pi_k > 0 $, $\mathcal{K}$ is a finite number, $\mu_k' = w_{\mathcal{A}}^T \, X_{\mathcal{A}}^* + w_{\mathcal{B}}^T \, \boldsymbol{\mu_k}$, and $\sigma_k'^2 = w_{\mathcal{B}}^T \, \boldsymbol{\Sigma_k} \, w_\mathcal{B}$.

\begin{proof}
Similar to the proof of Corollary~\ref{cor:adi-in-VFLR}, for any distribution of $X_{\mathcal{B}}$, we use Gaussian mixture model and Expectation Maximization to approximate its density function $p(X_{\mathcal{B}})$ as:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        p(X_{\mathcal{B}}) \approx \sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N}(X_{\mathcal{B}} | \boldsymbol{\mu_k}, \boldsymbol{\Sigma_k}) \; ,
    \end{aligned}
\end{equation}
\normalsize

\noindent where $ \sum_{k=1}^{\mathcal{K}} \pi_k = 1$, $ \pi_k > 0 $, $\mathcal{K}$ is a finite number, $\boldsymbol{\mu_k} \in \mathbb{R}^{d_2}$ and $\boldsymbol{\Sigma_k} \in \mathbb{R}^{d_2 \times d_2}$. 
Similarly, if $p(X_{\mathcal{B}})$ is highly discrete, we can approximate it by taking $\boldsymbol{\Sigma_k} \rightarrow \boldsymbol{0}$. 

For fixed $X_{\mathcal{A}}^*$, let $Y = w_{\mathcal{A}}^T
\, X_{\mathcal{A}}^* + w_{\mathcal{B}}^T \, X_{\mathcal{B}}$, $\mu_k' = w_{\mathcal{A}}^T
\, X_{\mathcal{A}}^* + w_{\mathcal{B}}^T \, \boldsymbol{\mu_k}$, and $\sigma_k'^2 =
w_{\mathcal{B}}^T \, \boldsymbol{\Sigma_k} \, w_\mathcal{B}$. Then, $p(Y) =
\sum_{k=1}^{\mathcal{K}} \pi_k \, \mathcal{N} (Y | \mu_k', \sigma_k'^2)$. We have: 

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y | Y > 0) = \sum_{k=1}^{\mathcal{K}} \pi_k \, (\mu_k' + \sigma_k' \frac{\phi(\frac{\mu_k'}{\sigma'_k})}{\Phi(\frac{\mu_k'}{\sigma_k'})})
    \end{aligned}
    \label{formula:e-cond}
\end{equation}

\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathcal{P} (Y > 0) = \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'})
    \end{aligned}
    \label{formula:p-cond}
\end{equation}
\normalsize
And we get the expected central coordinator output:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} \, &(f(X_{\mathcal{A}}^*, X_{\mathcal{B}})) = \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y | Y > 0) \times \mathcal{P} (Y > 0) \\
        =& (\sum_{k=1}^{\mathcal{K}} \pi_k \, (\mu_k' + \sigma_k' \frac{\phi(\frac{\mu_k'}{\sigma'_k})}{\Phi(\frac{\mu_k'}{\sigma_k'})}))
           \, (\sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'}))
    \end{aligned}
    \label{formula:e-relu}
\end{equation}
\normalsize
The variance of the truncated mixture Gaussian distribution is:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} & (Y | Y > 0) 
        = \sum_{k=1}^{\mathcal{K}} \pi_k^2 \, \sigma_k'^2(1 - \frac{\mu_k'}{\sigma_k'} \frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})} - (\frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})})^2)
    \end{aligned}
    \label{formula:v-Y}
\end{equation}
\normalsize

According to \E~\ref{formula:e-cond}, \ref{formula:p-cond}, \ref{formula:e-relu} and \ref{formula:v-Y}, we have:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y^2 | Y > 0) 
        = \, \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y | Y > 0) + (\mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y | Y > 0))^2
        % &= \mu'^2 + \sigma'^2 + \mu' \sigma' \frac{\phi(-\frac{\mu'}{\sigma'})}{1 - \Phi(-\frac{\mu'}{\sigma'})}
        % =& \sum_{k=1}^{\mathcal{K}} \pi_k^2 \, \sigma_k'^2(1 - \frac{\mu_k'}{\sigma_k'} \frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})} - (\frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})})^2)
        % + (\sum_{k=1}^{\mathcal{K}} \pi_k \, (\mu_k' + \sigma_k' \frac{\phi(\frac{\mu_k'}{\sigma'_k})}{\Phi(\frac{\mu_k'}{\sigma_k'})}))^2
    \end{aligned}
    \label{formula:e-squareY}
\end{equation}
\normalsize

\noindent Therefore, the variance of the coordinator model's output is:

\scriptsize
\setlength{\belowdisplayskip}{2pt} \setlength{\belowdisplayshortskip}{2pt}
\setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
\begin{equation}
    \begin{aligned}
        \mathbb{V}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} &(f(X_{\mathcal{A}}^*,X_{\mathcal{B}})) = \,
        \mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} (Y^2 | Y > 0) \times \mathcal{P} (Y > 0) 
        \\ & \qquad \qquad \qquad \qquad \, -(\mathbb{E}_{X_{\mathcal{B}} \in D_{\mathcal{B}}} \, (f(X_{\mathcal{A}}^*, X_{\mathcal{B}})))^2\\
        =& (\sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'})) \, 
        (\sum_{k=1}^{\mathcal{K}} \pi_k^2 \, \sigma_k'^2(1 - \frac{\mu_k'}{\sigma_k'} \frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})} - (\frac{\phi(\frac{\mu_k'}{\sigma_k'})}{\Phi(\frac{\mu_k'}{\sigma_k'})})^2) \\
        & + (\sum_{k=1}^{\mathcal{K}} \pi_k \, (\mu_k' + \sigma_k' \frac{\phi(\frac{\mu_k'}{\sigma'_k})}{\Phi(\frac{\mu_k'}{\sigma_k'})}))^2
        (1 - \sum_{k=1}^{\mathcal{K}} \pi_k \, \Phi(\frac{\mu_k'}{\sigma_k'})))
    \end{aligned}\qedhere
    \label{formula:v-relu}
\end{equation}
\normalsize
    
\end{proof}

==> related.tex <==
% \vspace{-5pt}
\section{Related Work}
\label{sec:related}
% \vspace{-5pt}

\noindent \textbf{Federated Learning.}~Horizontal federated learning 
was introduced to deliver a privacy-preserving solution for distributed machine
learning~\cite{mcmahan2017communication}, where instead of sharing the training
data, clients only share the model updates. The concept of federated learning is
further extended into a vertical
paradigm~\cite{hardy2017private,nock2018entity,yang2019federated}, in which
clients share datasets of distinct feature spaces but with the same ID space.
% Envisioning that federated learning is impeded by practical challenges, such as
% expensive communication and potentially non-IID data across different clients,
% several
% techniques~\cite{karimireddy2020scaffold,t2020personalized,he2020fedml,khan2020federated}
% have been proposed to reduce the communication cost such as using update
% quantization~\cite{konevcny2016federatedb,amiri2020federated}, fine-tuning
% homomorphic encryption precision~\cite{zhang2020batchcrypt}, and optimizing
% non-IID data~\cite{chai2020fedat,wang2020optimizing,mhaisen2020analysis}.

\noindent \textbf{Attacks on Federated Learning.}~Existing research
has demonstrated the feasibility of launching representative deep learning model
attacks, such as backdoor and reconstruction attacks, toward the federated
learning scheme. Nevertheless, most existing works either attack
HFL~\cite{chai2019towards,bagdasaryan2018backdoor,bhagoji2019analyzing,xie2019dba,sun2019can,wang2020attack,wang2019beyond,fang2020local,fung2020limitations,tolpegin2020data,nasr2019comprehensive},
or launch completely different attack schemes toward
VFL~\cite{liu2020backdoor,luo2020feature,weng2020privacy} (e.g., inferring
private data of victim participants).
% For instance, Bagdasaryan et
% al.~\cite{bagdasaryan2018backdoor} replaced the global model with a malicious
% local model by scaling up the attacker's updates, thus enabling the modeling of
% backdoor attacks in one iteration of the model update. Bhagoji et
% al.~\cite{bhagoji2019analyzing} propose a model poisoning attack by controlling
% a few malicious agents and thus inducing the central model to misclassify the
% chosen inputs. In addition, Xie et al.~\cite{xie2019dba} exploit the distributed
% nature of the federated learning framework by decomposing a backdoor trigger
% into multiple local patterns and embedding each local pattern into the training
% set of an adversarial client.
%A recent unpublished work~\cite{weng2020privacy}
%proposes privacy leakage attacks which explicitly manipulate several bits of the
%gradients. In contrast, we aim to control the joint VFL inference using ADIs in
%a stealthy manner.
In contrast, we propose a novel attack scheme that enables attackers to control
VFL joint prediction towards his will, extensively diminish others'
contribution and hog rewards that are used to incentivize participants. 
% These
% underlie the key novelty of our work.

\noindent \textbf{Hardening Federated Learning.}~Bonawitz et
al.~\cite{bonawitz2017practical} introduce secure aggregation to defeat a
semi-honest host and the dropout of arbitrary users.
Pillutla~\cite{pillutla2019robust} proposes a robust aggregation scheme toward
corrupted client updates. FoolsGold identifies sybil-based poisoning attacks
based on the client updating
diversity~\cite{fung2018mitigating}.~\cite{li2019fair} enhances the fairness of
resource allocation in HFL. Holistically, our present study assesses the unfair
contribution of VFL participants and the security implications. We leave it as
one future work to explore practical mitigation of the exposed ADIs.

